Compressing Neural Networks with the Hashing Trick

As deep nets are increasingly used in applications suited for mobile devices, a fundamental dilemma becomes apparent: the trend in deep learning is to grow models to absorb ever-increasing data set sizes; however mobile devices are designed with very little memory and cannot store such large models. We present a novel network architecture, HashedNets, that exploits inherent redundancy in neural networks to achieve drastic reductions in model sizes. HashedNets uses a low-cost hash function to randomly group connection weights into hash buckets, and all connections within the same hash bucket share a single parameter value. These parameters are tuned to adjust to the HashedNets weight sharing architecture with standard backprop during training. Our hashing procedure introduces no additional memory overhead, and we demonstrate on several benchmark data sets that HashedNets shrink the storage requirements of neural networks substantially while mostly preserving generalization performance.

==> content/discuss_old.tex <==
%!TEX root=../hashnn_main.tex

\newcommand{\bfy}[0]{{\textbf y}}

\section{Discussion}

We demonstrate that \abbrev{} is an unbiased approximation to the original fully-connected neural network.
For this attempt, we show the strong connection between \abbrev{} and the feature hashing trick proposed by \citet{weinberger09feature}. Due to this connection, \abbrev{} enjoys all the associated mathematical properties of feature hashing.

\subsection{Intuition}
To get the intuition, let's take a detour and cope with a classification dataset where a sample $\bx\in \mR^D$ has multiple labels $\bfy\in \mR^p$. The most straight way to address this problem is that we train $p$ different classifiers to fit $p$ different targets, \emph{i.e.} $y_i=f(\bW_i^\top \bx)$ where $\bW_i\in \mR^D$ is the weight vector for classifier $i$ and $f$ is a function such as sigmoid function in the case of logistic regression. The hashing trick suggests that instead of learning classifiers on $\bx$ which might be a high-dimensional vector, we can first hash the feature vector $\bx$ to a lower-dimensional representation $\phi(\bx)$ and then the classifiers could learn on top the representations, \emph{i.e.} $y_i=f(\bW_i^{\prime\top}  \phi(\bx))$ where $\bW_i^{\prime\top}$ is the new weight vector for classifier $i$. 

Inspired by the feature hashing trick for multi-task learning~\cite{weinberger09feature}, we can also hash the feature vector $\bx$ to get $p$ different new representations using $p$ different hash functions, and learn a unique weight vector $\bv$ jointly on these $p$ different new feature vectors, \emph{i.e.} $y_i=f(\bv^\top \phi_i(\bx))$ where $\phi_i(\cdot)$ is an independent hash function for $i=1,\cdots,p$.
Thanks to the property of approximate orthogonality~\cite{weinberger09feature}, if $\phi_i(\cdot)$ follows the formulation in Eq. \eqref{eq.feature_hashing_kwq}, we could get an unbiased estimate of the original $\bW_i^\top \bx$, \emph{i.e.} $\bv^\top \phi_i(\bx)\approx \bW_i^\top \bx$. In this way, a joint weight vector $\bv$ is empowered with the ability of achieving $p$ different learning goals. Most importantly, we can control the size of model parameters with ease by simply adjusting the length of $\bv$.

\subsection{Connecting \abbrev{} to Feature Hashing}
\label{sec.connection_to_hash}

We show that \abbrev{} model has a strong connection to feature hashing. Specifically, the proposed \abbrev{} model is equivalent to hashing neurons in layer $l$ into a joint hash space $n^{l+1}$ times with different hash functions, and then learning the parameter vector $\bv^l$ jointly. 


We describe \abbrev{} from the perspective of feature hashing in neural network. To get the value of neuron $i$ in layer $l+1$, we first hash the neurons in layer $l$ with hash mapping function $\phi_i^l (\cdot):\mR^{n^l}\rightarrow \mR^{K^l}$, and then apply the parameter vector $\bv^l$ on the hashed representation. Specifically, $\ai{l+1}=f( \zi{l+1} )$ and we have that
\begin{equation}
	\zi{l+1} = <\bv^{l}, \phi_i^l (\al{l}) >
	\label{eq.fhash_output}
\end{equation}
where $\phi_i^l (\al{l})$ is the resulting vector of hashing $\al{l}$. Please note the subscript $i$ since there are $n^{l+1}$ number of hash functions and they are independent from each other. But there's only one single weight vector $\bv^{l}$ in layer $l$. Both $\wl{l}$ and $\phi_i^l (\al{l})$ are $K^l$ dimensional vectors where $K^l$ is the number of hash buckets in layer $l$. Following Eq. \eqref{eq.feature_hashing_kwq}, the $k^{th}$ element of $ \phi_i^l (\al{l})$, \emph{i.e.} $\phi_{i,k}^l(\al{l})$, is the sum of variables hashed into bucket $k$ up to a sign factor:
\begin{equation}
	\phi_{i,k}^l (\al{l}) = \sum_{j:h_i^l(j)=k} \xi_i^l(j) a_j^l
	\label{eq.myhash}
\end{equation}
where $h_i^l:\mathbb{N}\rightarrow \{1,\cdots,K^l\}$ and $\xi_i^l:\mathbb{N}\rightarrow \{\pm 1\}$ are independent hash functions. 


%Figure \ref{fig:hashnn2} illustrates the architecture of \abbrev{}-2.

% \begin{figure}
%     \centerline{
%     \includegraphics[width=0.5\textwidth]{figures/hashnn_architecture.pdf}
% 	}
%     \caption{Illustration of \abbrev{}-2 network. Each layer in \abbrev{}-2 could be further decomposed into two phases, where the first phase is feature hashing (blue edges) and the second one is a linear model (black edges). In this example, during feature hashing phase the input vector $\al{l}$ is hashed three times since there are 3 output neurons in layer $l+1$. Since Eq. \eqref{eq.myhash} could be considered a linear mapping, The blue edges describe the computation of feature hashing in a fashion of linear multiplication where the connection is specified by hash function $h_i^l$ and the weight of each edge is either 1 or -1 depending on the value of $\xi^l_i$. The second phase is a standard linear mapping except that the parameter vector $\bv^l$ is shared among all hashed inputs.}
%     \label{fig:hashnn2}
% \end{figure}

We show that the neural network defined by Eq. \eqref{eq.fhash_output} has the same outputs, error terms and gradients over parameters $\bv^l$ as \abbrev{}, and thus they are equivalent.

\paragraph{Same output.}
We show that Eq. \eqref{eq.fhash_output} is equivalent to Eq. \eqref{eq.hash_output}.
Starting from Eq. \eqref{eq.fhash_output}, we have that
\begin{eqnarray}
	z_i^{l+1} &=&  \sum_k^{K^l} v_k^{l} \phi_{i,k}^l (\al{l}) \label{eq.same_output_0} \\
	&=&  \sum_k^{K^l} v_k^{l} \sum_{j:h_i^l(j)=k} \xi_i^l(j) a_j^l \label{eq.same_output_1} \\
	&=& \sum_j^{n^l} v_{h^l_i(j)}^{l} \xi_i^l(j) a_j^l \label{eq.same_output_2}
\end{eqnarray}
where Eq. \eqref{eq.same_output_1} is obtained by substituting Eq. \eqref{eq.myhash} into Eq. \eqref{eq.same_output_0}. We can see that Eq. \eqref{eq.same_output_2} is identical to Eq. \eqref{eq.hash_output}.

\paragraph{Same error term.}
We first propagate the error from layer $l+1$ to $\phi_{j}^{l}(\ba^l)$. Denote the error of $k^{th}$ unit of $\phi_{j,k}^{l}(\ba^l)$ as $\delta_{j,k}^{l+0.5}$. Following the chain rule, we have
\begin{equation}
	\delta_{j,k}^{l+0.5} =  v_{k}^l \delta_j^{l+1} 
	\label{eq.middle_layer_error}
\end{equation}
To get the error terms of layer $l$, we further propagate error in Eq. \eqref{eq.middle_layer_error} back to layer $l$ as follows
\begin{eqnarray}
	\delta_i^l &=& (\sum_j^{n^{l+1}} \xi_j^l(i) \delta_{j,h_j^l(i)}^{l+0.5} ) f^\prime(z_i^l) \label{eq.same_error_1}\\
	           &=& (\sum_j^{n^{l+1}} \xi_j^l(i) v_{h_j^l(i)}^l \delta_j^{l+1}) f^\prime(z_i^l) \label{eq.same_error_2}
\end{eqnarray}
where Eq. \eqref{eq.same_error_1} is a direct result of chain rule in back propagation. Substituting Eq. \eqref{eq.middle_layer_error} into Eq. \eqref{eq.same_error_1}, we can obtain Eq. \eqref{eq.same_error_2}, which is identical to Eq. \eqref{eq.error_term}.


\paragraph{Same gradient over weights.}
According to the chain rule and the relation between $z_i^{l+1}$ and $\bv^l$, we have that the gradient over $\bv^{l}$ is as follow:
\begin{equation}
	\gradL{v_k^l} = \sum_{i=1}^{n^{l+1}} \phi_{i,k}^{l} (\ba^l) \delta_i^{l+1} = \sum_{i=1}^{n^{l+1}} \sum_{j:h_i^l(j)=k} \xi_i^l(j) a_j^l \delta_i^{l+1}
	\label{eq.hash2_gradient}
\end{equation}
where the last equality can be obtained by combining with Eq. \eqref{eq.myhash}. We can see that Eq. \eqref{eq.hash2_gradient} is exactly same as Eq. \eqref{eq.grad3}.
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\blacksquare$

\subsection{Properties}
\paragraph{Unbiased approximation.} 
\abbrev{}, as shown in Section \ref{sec.connection_to_hash}, is equivalent to doing feature hashing on neurons. Due to the property of approximate orthogonality~\cite{weinberger09feature}, we can conclude that \abbrev{} is an unbiased approximation to the original fully connected network, \emph{i.e.} $\bv^{l\top} \phi_i^l(\ba^l)\approx \bW_i^{l\top} \ba^l$.

\paragraph{Sparsity.} 
Feature hashing works best on sparse feature vectors since the feature collision caused by hashing is minimized. In place of sigmoid and Tanh function, today rectifier linear unit (ReLu)~\cite{glorot2011deep} has been widely used as the activation function for neural networks. Besides its simplicity and superior accuracy performance, it offers many good properties. It allows a neural network to easily achieve sparse representation on each hidden layer which makes \abbrev{} a great fit for compressing neural network. This benefit could be further enhanced when sparsity inducing norm is involved.

\paragraph{Other kinds of neural networks.}
Though focusing on general fully connected network in this paper, the technique of \abbrev{} could be extended to all kinds of neural networks, such as convolutional neural network and auto-encoder.







